Footprints of Higher-Dimensional Decaying Black Holes

We review the current results for the emission of Hawking radiation by a higher-dimensional black hole during the Schwarzschild and the spin-down phases. We discuss particularly the role of the angular variation of the emitted radiation on the brane during the latter phase, the radiation spectra for gravitons in the bulk, and the effect of the mass of the emitted particles in determining the bulk-to-brane energy balance.

==> rjp_mathdefs.tex <==
%This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
% that are currently in use and accepted by Romanian Journal of Physics.

%Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

%Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
\providecommand{\pd}{\ensuremath{\partial}}
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}

%bras and kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
%the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}

%Commands for multiple indexes around a central token #1
%The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
%the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
%that it diminishes the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}
\newcommand{\fdbu}[3]{{\!\;}_{#2}\!#1^{#3}}
\newcommand{\fubd}[3]{{\!\;}^{#2}\!#1_{#3}}

%put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}

%A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

